Evolving Scientific Discovery by Unifying Data and Background Knowledge with AI Hilbert

The discovery of scientific formulae that parsimoniously explain natural phenomena and align with existing background theory is a key goal in science. Historically, scientists have derived natural laws by manipulating equations based on existing knowledge, forming new equations, and verifying them experimentally. In recent years, data-driven scientific discovery has emerged as a viable competitor in settings with large amounts of experimental data. Unfortunately, data-driven methods often fail to discover valid laws when data is noisy or scarce. Accordingly, recent works combine regression and reasoning to eliminate formulae inconsistent with background theory. However, the problem of searching over the space of formulae consistent with background theory to find one that best fits the data is not well-solved. We propose a solution to this problem when all axioms and scientific laws are expressible via polynomial equalities and inequalities and argue that our approach is widely applicable. We model notions of minimal complexity using binary variables and logical constraints, solve polynomial optimization problems via mixed-integer linear or semidefinite optimization, and prove the validity of our scientific discoveries in a principled manner using Positivstellensatz certificates. The optimization techniques leveraged in this paper allow our approach to run in polynomial time with fully correct background theory under an assumption that the complexity of our derivation is bounded), or non-deterministic polynomial (NP) time with partially correct background theory. We demonstrate that some famous scientific laws, including Kepler's Third Law of Planetary Motion, the Hagen-Poiseuille Equation, and the Radiated Gravitational Wave Power equation, can be derived in a principled manner from axioms and experimental data.

==> table.tex <==

\begin{table}[h]
  \caption{\color{blue}Comparison of {AI-Hilbert} with state-of-the-art discovery methods in terms of ability to recover scientific laws from background theory and experimental data. {AI-Hilbert} recovers both scientific laws by combining experimental data and background theory via polynomial optimization, while state-of-the-art approaches fail at discovering both. 
  \newline
  \cri{SANJEEB check the point $^\ast$ below} \newline
  $^\ast$  This symbol next to \checkmark denotes success up to a constant approximation. This is because the methods considered from the literature are data-driven, and thus cannot exactly derive constants associated with scientific laws. Instead, they usually group information concerning multiple constants into one that is less interpretable. For instance, consider the Compton Scattering problem (\ref{ssec:compton}), the correct formula is
  $l_2  = l_1 + \frac{h}{m_e  c }(1 - cos(\theta))$
  while a data-driven method can only derive 
  $l_2  = l_1 + k(1- cos(\theta))$ (where $k$ is a real number), since, $m_e$, $c$, and $h$ are all constants.
  Moreover sometimes integers of fractions are reported with a small numerical error (e.g., $1,001$ or $0.999$ instead of $1$).
  \newline
  \cri{LIOR check the point $^\diamond$ below} \newline
  $^\diamond$ To generate data for this problem, we varied the mass values of both the pion and the muon. These variations were intended to mimic small differences in the observed values of the masses, rather than altering the actual values across a broad range of values. 
  \newline
  $^\dagger$ Inequalities are not supported by the methods from the literature that we benchmarked against.
  }
  \centering\footnotesize
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c l c c c c c c}
    \toprule
     Data & & {AI-Hilbert}  & AI-Descartes \cite{cornelio2021ai} & AI-Feynman \cite{udrescu2020ai}  & PySR \cite{cranmer10pysr} & BMS \cite{guimera2020bayesian}\\
    \midrule
    S & [\ref{ssec:Hagen}] Hagen Poiseuille  & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{red}{???} & \textcolor{red}{???} & \textcolor{red}{$\text{\xmark}$} &  \textcolor{red}{$\text{\xmark}$} \\
    R & [\ref{ssec:einstein}] Relat. Time Dilat.  & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{red}{$\text{\xmark}\phantom{0}$} & \textcolor{red}{$\text{\xmark}$}& \textcolor{red}{$\text{\xmark}$}&  \textcolor{red}{$\text{\xmark}$} \\
    R & [\ref{ssec:kepler}] Kepler's 3 Law & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{orange}{$\text{\checkmark}^\ast$}  & \textcolor{red}{$\text{\xmark}$} & \textcolor{teal}{$\text{\checkmark}$} &  \textcolor{red}{$\text{\xmark}$}  \\
    S & [\ref{ssec:gravwaves}] Gravitational Wave Power & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{red}{???} & \textcolor{red}{???} & \textcolor{red}{$\text{\xmark}$} &  \textcolor{red}{$\text{\xmark}$} \\
    S & [\ref{ssec:bell}] Bell inequalities$^\dagger$& \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{red}{$\text{\xmark}\phantom{0}$} & \textcolor{red}{$\text{\xmark}$} & \textcolor{red}{$\text{\xmark}$} & \textcolor{red}{$\text{\xmark}$}  \\
    
    \midrule
    S & [\ref{ssec:fsrd}] {I.15.10} FSRD & \textcolor{teal}{$\text{\checkmark}$} & \textcolor{orange}{$\text{\checkmark}^\ast$} & \textcolor{red}{$\text{\xmark}$} & \textcolor{red}{$\text{\xmark}$} & \textcolor{red}{$\text{\xmark}$}  \\
    S & [\ref{ssec:fsrd}] {I.27.6} FSRD & \textcolor{red}{???}
    & \textcolor{orange}{$\text{\checkmark}^\ast$} & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} & \textcolor{teal}{$\text{\checkmark}$} & \textcolor{red}{$\text{\xmark}$}  \\
    S & [\ref{ssec:fsrd}] {I.34.8} FSRD & \textcolor{red}{???}
    & \textcolor{teal}{$\text{\checkmark}$} \phantom{0} & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} & \textcolor{teal}{$\text{\checkmark}$}&  \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$}  \\
    S & [\ref{ssec:fsrd}] {I.43.16} FSRD & \textcolor{teal}{$\text{\checkmark}$} & \textcolor{orange}{$\text{\checkmark}^\ast$}  & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} & \textcolor{teal}{$\text{\checkmark}$}& \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$}  \\
    S & [\ref{ssec:fsrd}] {II.10.9}  FSRD & \textcolor{teal}{$\text{\checkmark}$} &\textcolor{orange}{$\text{\checkmark}^\ast$} & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$}& \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$}  \\
    S & [\ref{ssec:fsrd}] {II.34.2} FSRD & \textcolor{teal}{$\text{\checkmark}$} & \textcolor{orange}{$\text{\checkmark}^\ast$}  & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$}   \\
    
    \midrule
    S & [\ref{append:relcollision}] Inelastic Relativ. Collision 
    & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{orange}{$\text{\checkmark}^\ast$}  &  \textcolor{red}{$\text{\xmark}$}
    & \textcolor{red}{$\text{\xmark}$} & \textcolor{red}{$\text{\xmark}$}  \\
    S & [\ref{ssec:pion}] Decay of Pion$^\diamond$
    & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{orange}{$\text{\checkmark}^\ast$}  & \textcolor{red}{$\text{\xmark}$}
    & \textcolor{red}{$\text{\xmark}$} &  \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} \\
    S & [\ref{ssec:lightscattering}] Radiation Damping
    & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{red}{$\text{\xmark}\phantom{0}$}  &  \textcolor{red}{$\text{\xmark}$}
    & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$}  \\
    S & [\ref{ssec:escapevelocity}] Escape Velocity
    & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{teal}{$\text{\checkmark}\phantom{0}$}  &  \textcolor{orange}{$\text{\checkmark}^\ast$}
    & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$}  \\
    S & [\ref{ssec:halleffect}] Hall Effect
    & \textcolor{teal}{$\text{\checkmark}$}  & \textcolor{orange}{$\text{\checkmark}^\ast$}  & \textcolor{red}{$\text{\xmark}$}
    & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} &  \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} \\
    S & [\ref{ssec:compton}] Compton Scattering
    & \textcolor{teal}{$\text{\checkmark}$}  &  \textcolor{orange}{$\text{\checkmark}^\ast$} & \textcolor{orange}{$\text{\checkmark}^\ast$}
    & \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} &  \phantom{0}\textcolor{orange}{$\text{\checkmark}^\ast$} \\
    \bottomrule  
  \end{tabular}}
  \label{tab:comparison_scientificlaws}
\end{table}
